SwinAD: Multi-stage feature reconstruction for unsupervised industrial anomaly detection

Industrial anomaly detection aims to identify and localize defective regions without relying on exhaustive annotations of all possible defect types. Although recent unsupervised methods have achieved strong performance, most are primarily designed for single-class settings and often struggle in multi-class scenarios, where diverse normal patterns may lead to over-generalization and reduce the discriminative capability between normal and anomalous regions. In this paper, we propose SwinAD, a reconstruction-based framework for multi-class unsupervised anomaly detection that leverages a frozen pretrained Swin Transformer V2 encoder and a feature diversity-preserving reconstruction decoder. The hierarchical encoder provides semantically rich multi-scale features, while stage-wise bottleneck modules with dropout prevent trivial identity mapping and encourage robust reconstruction of normal patterns. To further improve localization, we introduce a feature diversity-preserving reconstruction framework that maintains complementary reconstruction hypotheses instead of relying on a single decoding branch. The discrepancies between encoder features and the two reconstructed features are then aggregated across multiple scales to produce the final anomaly map. Experiments conducted on three industrial anomaly detection benchmarks, including MVTec AD, VisA, and Real-IAD, demonstrate that SwinAD achieves competitive image-level performance and strong pixel-level localization accuracy, with particularly notable improvements in pixel-level AP and 1 on MVTec AD. These results indicate that combining hierarchical Swin features with diverse multi-scale reconstruction substantially improve pixel-level localization in multi-class unsupervised anomaly setting.

==> Method.tex <==
\subsection{SwinTransform Encoder}
For the image encoder, we employ a Swin Transformer V2 model \cite{liu2022swin}, denoted as $\phi_{S}(·)$. Leveraging its hierarchical attention architecture and shifted window mechanism, SwinV2 facilitates effective multi-scale feature extraction. This design significantly enhances the model's capacity to capture both fine-grained local details and broad global contexts within image. The encoder processes an input image $I \in \mathbb{R}^{3 \times H \times W}$ through a series of stages involving self-Attention with shifted-Window mechanism. Unlike the standard ViT, SwinV2 produces multi-scale feature maps; however, we specifically utilize the output from the final stage, denoted as $\phi_{S}(I) = [f_1, f_2, \dots, f_N] \in \mathbb{R}^{N \times D}$. Here, $f_p \in \mathbb{R}^D$ represents the output embedding for a spatial grid cell $p \in [1, \dots, N]$, where $N = \frac{H}{32} \times \frac{W}{32}$ typically. Since Swinv2 inherently performs global average pooling rather than using a $[CLS]$ token, we derive the global representation $c \in \mathbb{R}^D$ by aggregating the final feature map to ensure compatibility with downstream tasks. 
\subsection{Loss funtion}
The final training objective combine the 
\begin{equation*}
    \mathcal{L} = \sum_{i=1}^{K} (L^k_{local} + \alpha L^k_{global})
\end{equation*}
where $\alpha$ 

\subsection{Anomaly Map Estimation}

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

%% Keep related quantitative and qualitative floats grouped.
\usepackage{placeins}

